Soft Robotic Mannequin: Design and Algorithm for Deformation Control

This paper presents a novel soft robotic system for a deformable mannequin that can be employed to physically realize the 3D geometry of different human bodies. The soft membrane on a mannequin is deformed by inflating several curved chambers using pneumatic actuation. Controlling the freeform surface of a soft membrane by adjusting the pneumatic actuation in different chambers is challenging as the membrane's shape is commonly determined by the interaction between all chambers. Using vision feedback provided by a structured-light based 3D scanner, we developed an efficient algorithm to compute the optimized actuation of all chambers which could drive the soft membrane to deform into the best approximation of different target shapes. Our algorithm converges quickly by including pose estimation in the loop of optimization. The time-consuming step of evaluating derivatives on the deformable membrane is avoided by using the Broyden update when possible. The effectiveness of our soft robotic mannequin with controlled deformation has been verified in experiments.

==> tex/textConclusion.tex <==
\section{Conclusion \& Discussion}

\subsection{Conclusion}
\label{sec:Conclusion}
\par In this paper, we present a method to actuate the deformable membrane to approximate target 3D continuous shape by model-free Coarse-to-fine solver with ICP. As our method could nicely close-loop control the 3D shape of continuous surface, which to the best of our knowledge, has not been realized by others in physical experiments.

\par Approximating captured surface to target surface shape is a high DoF problem because the description of surface distance needs large numbers of variables. In order to solve this, we reduced the dimension of data by grouping distances between re-sample points (on fitted B-spline surface from raw point cloud) and closest target points.

\par Considering orientation of target shape might not be perfectly aligned with current shape captured by scanner, we looked for the help of ICP to correct the orientation and translation of target shape, and also provide some extra iteration directions, which also makes our problem not simply inverse kinematics (IK) problem. After we formulated our approximation problem into two kinds of problems: energy minimization problem and root-finding problem, we adopt gradient descent method with gradient estimated by forward difference where we slightly change the value of actuation and record respect camera data. Even though the accuracy of gradient descent method is relatively promising, but the time needed for estimating gradient is high, so we invited Broyden Update method (with respect to root-finding problem) to speed up the iteration.
Last but not least, considering the limits of actuation range, barrier energy is introduced in our objective in Coarse phase to avoid hitting actuation boundary as much as possible, while we remain the same objective in fine phase to chase iteration convergence. 

\subsection{Discussion}
\Jun{discuss about the time-consuming gradient estimation due to hysteresis effect}
\subsubsection{Role of ICP}
\par In our experiments, ICP plays an important role in our control algorithm due to the following reasons:

\begin{itemize}
    \item Initial alignment of captured surface and target surface could be not critically reasonable, ICP algorithm would gradually adjust the orientation and translation of target shape to improve the approximation.
    \item As mentioned in \ref{sec:Conclusion}, ICP would provide extra directions of iteration so that converging speed would be fast and stable. It truly eliminates the gap of our control algorithm from reality.
\end{itemize}

\par However, ICP algorithm deployed in our solve does have some shortcomings. For example, the initial orientation and translation of target shape with respect to captured shape is the most critical, otherwise the target shape would be applied a totally wrong rigid transformation which means the iteration falls into a local minimal and it just gets stuck at around that point. This could be seem in (\Jun{Please add more chapter reference here}).

\subsubsection{Objective Selection}
\par In our solver, objective is defined as the distance sum of fitted surface points from captured raw data and respect closest target fitted surface points instead of simply the sum of fitted control points and target control points. The reasons why we do this could be stated as following:
\begin{itemize}
    \item When we choose the latter, the fitted control point and the respect target control point would slip a little bit at the direction of surface plane. This is because we could not guarantee equality of surface dimensions of captured surface and target surface.
    So the distance vector of two control points would be added in the direction of u and v direction. \Jun{Should add the slipped demonstration fig here.}
    \item However, If the distance is defined between captured fitted surface point and closest target fitted point, the problem would be perfectly solved and the restriction that we need to make sure the dimension of target surface and captured surface becomes the same no longer exists.
\end{itemize}

\charlie{Slow gradient evaluation (12.5 sec. per actuation) caused by material hysteresis.}


\subsubsection{Future Works}
\par In this paper, plane chamber design is selected and rod array is also parallel which would make the approximation a little unreal especially at around the boundary of chamber. So design of curved chamber would be proposed and validated. Also, this vision-based algorithm needs real-time and high-precision visual stream as feedback information, which would limit the application situations (e.g. When light condition is not reasonable). In the future, we would design some embedded sensors to capture the deformation information to replace the vision device used in this paper.


==> tex/textControlTheory.tex <==


\subsection{Discussion}
\subsubsection{Role of ICP}
\par In our experiments, ICP plays an important role in our control algorithm due to the following reasons:

\begin{itemize}
    \item Initial alignment of captured surface and target surface could be not critically reasonable, ICP algorithm would gradually adjust the orientation and translation of target shape to improve the approximation.
    \item As mentioned in \ref{sec:Conclusion}, ICP would provide extra directions of iteration so that converging speed would be fast and stable. It truly eliminates the gap of our control algorithm from reality.
\end{itemize}

\par However, ICP algorithm deployed in our solve does have some shortcomings. For example, the initial orientation and translation of target shape with respect to captured shape is the most critical, otherwise the target shape would be applied a totally wrong rigid transformation which means the iteration falls into a local minimal and it just gets stuck at around that point. This could be seem in (\Jun{Please add more chapter reference here}).

\subsubsection{Objective Selection}
\par In our solver, objective is defined as the distance sum of fitted surface points from captured raw data and respect closest target fitted surface points instead of simply the sum of fitted control points and target control points. The reasons why we do this could be stated as following:
\begin{itemize}
    \item When we choose the latter, the fitted control point and the respect target control point would slip a little bit at the direction of surface plane. This is because we could not guarantee equality of surface dimensions of captured surface and target surface.
    So the distance vector of two control points would be added in the direction of u and v direction. \Jun{Should add the slipped demonstration fig here.}
    \item However, If the distance is defined between captured fitted surface point and closest target fitted point, the problem would be perfectly solved and the restriction that we need to make sure the dimension of target surface and captured surface becomes the same no longer exists.
\end{itemize}


\subsubsection{Future Works}
\par In this paper, plane chamber design is selected and rod array is also parallel which would make the approximation a little unreal especially at around the boundary of chamber. So design of curved chamber would be proposed and validated. Also, this vision-based algorithm needs real-time and high-precision visual stream as feedback information, which would limit the application situations (e.g. When light condition is not reasonable). In the future, we would design some embedded sensors to capture the deformation information to replace the vision device used in this paper.


% \newpage
% ...Segmentation Page...
% \newpage
% \subsection{Preparation of Feature Points}
% \label{sec: FeaturePnts}
% \Jun{I am working on this paragraph: 0313}


% \Jun{I think maybe we should first define feature point in two vision system: Vicon Motion Capture System and Artec 3D Scanner.
% Then, we point out feature points including target feature points and real-time feature points. As for target feature points, we use B-spline surface fitting to down-sample the high-dimensional geometry information in both vision systems; As for real-time feature points, we use original data stream from Vicon Cam with gaussian filtering to become RT feature points. In Artec 3D Scanner, the input information is large scale, so we also use b-spline fitting to reduce the dimension of overall surface shape.}


% \JunReplace{}{In our setup, feature points could be classified into two classes: real-time feature points and target feature points. Also, there are two vision systems to provide real-time information. In Vicon Motion Capture System, we directly acquire data streaming from cameras and processed by guassian filtering. Another system is Artec 3D Scanner, the large-scale input data is not realistic to be directly used as feedback information because of the extreme high computation cost of processing raw data (e.g. acquiring, storing, filtering, comparing, ...), so we invite B-Spline surface fitting to reduce the dimension of surface geometry. This could not only reduce the difficulty of control, but also provide overall smooth surface shape with noise somehow being filtered out. Therefore, the deformable surface shape $\mathcal{M}$ can be describe as:
% \begin{equation}
%     x(u,v) = \sum_{i=0}^b \sum_{j=0}^h N_{i,p}(u) N_{j,q}(u)\mathbf{p}_{i,j}
% \end{equation}
% where the $N(\cdot)$ are B-spline basis functions of degree p and q, respectively. The control point position $\mathbf{p}_{i,j}$ is the actual value controlled in configuration space, which lower the dimension with $n = 3bh$. }



% \JunReplace{}{As for target feature points, if we are using Vicon Motion Capture System to acquire real-time information, we use processed B-Spline surface to become target shape. To be more precise, we use the point on the surface sharing same $(u,v)$ with the marker to become respect target points. The parameterization method is straightforward which comes from the relative position of marker with respect to the dimension of raw point cloud in $Region \ of\  Interest$ (ROI):} 

% \begin{equation}
% \label{Equ: para:1}
%     u = \frac{x - x_{min}}{x_{max}-x_{min}}
% \end{equation}

% \begin{equation}
% \label{Equ: para:2}
%     v = \frac{y - y_{min}}{y_{max}-y_{min}}
% \end{equation}


% \JunReplace{}{The equation of comparing the shape difference can be written as following:}

% \begin{equation}
% \small
% \label{Equ: shapeDifference:1}
%      \mathcal{O}(\mathcal{M}_t,\mathcal{M}_c) = 
%       \sum_{i\in S_{marker}}( x_i - x^*(u_i,v_i))^2 
% \end{equation}

% \JunReplace{}{Which could be detailedly written as:}

% \begin{equation}
% \small
% \label{Equ: shapeDifference:2}
%      \mathcal{O}(\mathcal{M}_t,\mathcal{M}_c) =\sum_{i\in S_{marker}}( x_i -  \sum_{i=0}^b \sum_{j=0}^h N_{i,p}(u_i) N_{j,q}(v_i)\mathbf{p}_{i,j})^2
% \end{equation}

% \JunReplace{}{
% If we are talking about using Artec 3D Scanner to be real-time information source, we use processed B-Spline control points as target feature points because the input real-time data is also B-Spline control points, the direct comparing of control points is a reasonable method to compare the difference of overall shape.}

% \JunReplace{}{With this method, we illustrate the difference between two mesh as an energy which computes:}

% \begin{equation} \label{eq:objective}
%     \mathcal{O}(\mathcal{M}_t,\mathcal{M}_c) = \sum_{i=0}^b \sum_{j=0}^h || \mathbf{p}_{i,j}^t - \mathbf{p}_{i,j}^c ||_F^2
% \end{equation}

% \JunReplace{}{Remember, in the shape difference, we always apply ICP first and then comparing the difference between target and real-time shape. So energy objective function should always include $(R, T)$ to represent this method.}



% \section{Experimental Validation }\label{secExperiment}

% we use processed B-Spline (captured from mannequin point cloud) as feature points to

% \section{Discussion}\label{secDiscussion}

% \subsection{Simulation of Mannequin Design}
% \Jun{Working on this paragraph}

% \Jun{Here, we should provide some details about source of female models.}
% \JunReplace{}{Firstly, we have chosen female templates from WebGL Model Generator(finish later) with different parameters describing characteristics of human models. }
% \JunReplace{}{In order to verify our mechanical design, finite element simulations about actuation applied to design are important, so lots of deformation simulations have been finished to verify and help improve our current design.}

% \JunReplace{}{In this section, simulation of mannequin design would be shown including chamber inflation and rod linear movement. After physical simulation, quantification of distance error between simulated membrane shape and target one would be examined, and its result would be visualized by mesh color map.}

% \JunReplace{}{
% In this paper, four female models shown in Fig \ref{fig:femaleModelAndMechanicalDesign} (a) are selected to be target template, and dark olive green points on the female model are in the Region of Interest (ROI) which would be matched as closely as possible by deformed membrane. In Fig\ref{fig:femaleModelAndMechanicalDesign} (b), initial and final design of our experimental setup has been shown. Left figure shows the initial design which contains two huge chest chambers and two waist chambers. However, after several simulations and optimizations, the chest chambers have been merged into one, and number of waist chamber has changed from two to three. More than that, restrictions of membrane inflation movements are added to our simulation by placing two stick obstacle near waist chambers to limit the movement of membrane in z direction.}

% \Jun{Here, start to show simulation results of initial design}
% \JunReplace{}{Fig [] shows simulation results of initial design by presenting color map of distance error between deformed surfaces and ROI of female templates. Maximum distance error of colormap is chosen to be 10 mm.}


% \Jun{Here, we need a figure to show four human models with selected area}
% \Jun{Second fig is about initial mechanical design and final mechanical design}
% \Jun{Third fig is about initial simulation results}
% \Jun{Forth fig is about final   simulation results}

% \begin{figure*}[h]
% \centering
% \includegraphics[width=\linewidth]{fig/paperFig-femaleAndDesign.png}
% \caption{ (a) are female models selected as targets, dark olive green points on the female model are in the Region of Interest (ROI) of our experiments. Figs in (b) are initial design and final design of our mannequin setup. \Jun{Will be polished later}
% }\label{fig:femaleModelAndMechanicalDesign}
% \end{figure*}

% \Jun{segmentation line}
% \newpage
% We remark the mannequin model with mesh representation as $\mathcal{M}$. The control goal is finding the control parameter (represented by vector $\mathbf{c} \in \mathbb{R}^m$) that makes the shape close to given target model shape $\mathcal{M}_t$. As Jacobian-based method is invited in our system, the Jacobian matrix $\mathbf{J} \in \mathbb{R}^{m \times n}$ needs to be computed and updated for each iteration. 

% Here $n$ is the dimention of the control parameters, which can be intuitively set as the coordinate of each vertex in the given target shape mesh $\mathcal{M}_t$. However, this can easily cause a large dimension that requires extreme high computation cost. Instead, in our method we invite the B-spline surface fitting to down-sampling the control variables into the b-spline surface control point, where the target and our current mesh are both fit with same dimension (as detailed in sec...). Therefore, the deformable surface shape $\mathcal{M}$ can be describe as:
% \begin{equation}
%     \mathbf{p}(u,v) = \sum_{i=0}^b \sum_{j=0}^h N_{i,p}(u) N_{j,q}(u)\mathbf{p}_{i,j}
% \end{equation}
% where the $N(\cdot)$ are B-spline basis functions of degree p and q, respectively. The control point position $\mathbf{p}_{i,j}$ is the actual value controlled in configuration space, which lower the dimension with $n = 3bh$. Meanwhile, 

% With this method, we illustrate the difference between two mesh as an objective function which computes
% \begin{equation} \label{eq:objective}
%     \mathcal{O}(\mathcal{M}_t,\mathcal{M}_c) = \sum_{i=0}^b \sum_{j=0}^h || \mathbf{p}_{i,j}^t - \mathbf{p}_{i,j}^c ||_F^2
% \end{equation}

% To best mimic the difference between two deformed status of the surface, we invite ICP to apply the rigid transformation to $\mathcal{M}_t$ and make it close to the current status. We can compute $\mathcal{M}_t^{r} = \mathbf{R}\mathcal{M}_t + \mathbf{t}$ and brings it to (\ref{eq:objective}).



% \Guoxin{Working on the algorithm now}









% Here we invite two 

% When give the initial control vector and shape status ($\mathbf{c}_0$ and 


% input of our method is the target shape model $\mathcal{M}_t$. We define the configuration space control parameter as 




% \subsection{Vision-based Objectives by Shape Difference}
% The goal of control pipeline is find the proper actuation parameter $\mathbf{c}$ which drives the deformable surface to certain shape that best mimic the given target input. To reach this goal, our control pipeline using gradient based iterative method to minimize the objective functions and update the control parameters iterative. An intutive way of define such shape difference between is by directly measure the difference of the control point position, which can be written as
% \begin{equation*}
%     f_{\mathbf{diff}}(\mathcal{P}^t,\mathcal{P}^c) = \sum_{i=0}^b \sum_{j=0}^h || \mathbf{p}_{i,j}^t - \mathbf{p}_{i,j}^c ||_F^2.
% \end{equation*}

% However, using such measurement didn't consider the initial position difference from the target shape and may brings a large variation in the transformation matrix, which can brings the system hard to converge. Here we invite \textit{iterative closest point} (ICP) algorithm to first transform the target point cloud $\mathcal{P}^t$ to a certain region to delineate the shape error from the rigid transformation. We mark the transformed target shape as $\mathcal{P}^{tr} = \mathbf{R}\mathcal{P}^t+\mathbf{t}$. \Guoxin{A figure should be added here.} Therefore, we can define the objective function for each iteration as
% \begin{equation} \label{eq:objective}
%     \mathcal{O}(\mathcal{P}^t,\mathcal{P}^c(\mathbf{c})) = \sum_{i=0}^b \sum_{j=0}^h || (\mathbf{R}\mathbf{p}_{i,j}^t + \mathbf{t}) - \mathbf{p}_{i,j}^c ||_F^2.
% \end{equation}

% \Guoxin{Add discussion here when to apply ICP, it should be using estimated Jacobian matrix cannot lower the objective values anymore.}

% In each iteration, after run the given control parameter in the physical system, we can compute the objective value of current vision-captured shape of deformable surface. To minimize this objectives in the efficient way, we invite gradient-based optimization method where the Jacobian Matrix $\mathbf{J} = d\mathbf{p}/d\mathbf{c}$ is used. We detail the method used to compute the Jacobian Matrix in the following section.

% \subsection{Estimation of Jacobian Matrix}
% For the computing of Jacobian, we conduct a hybird method to estimate it, with the balance of computational cost and efficiency. 

% \subsubsection{Jacobian by numerical difference}
% Firstly and most intuitive way of estimate the Jacobian matrix of the objective function is by numerical difference, where the k-th item of gradient vector can be written as
% \begin{equation} \label{eq:numericalJacobian}
%     \frac{\partial \mathcal{O}(\mathbf{c})}{\partial c_k} = \frac{\mathcal{O}(..., c_k+\Delta c, ...) - \mathcal{O}(..., c_k-\Delta c, ...)}{2 \Delta c}
% \end{equation}
% Notice that to compute the gradient in such way requires us to move each actuator individually in physical setup. Therefore in total $n$ times capture is needed, which is time-consuming. We we remark the Jacobian computed by this method as $\mathbf{J}_{num}$ and used for the initial Jacobian matrix computing scheme. To avoid such computing in real model, we brings another estimation method to fast compute the Jacobian.

% \subsubsection{Estimate Jacobian by Broyden's iteration}
% Based on the previous statutes of the system, Broyden's iteration~\cite{} can estimate the Jacobian matrix of our visual servoed control system. For the i-th iteration, when using the Jacobian $\mathbf{J}_i$ and searching step (discussed later) to find the control parameter incremental amount in the next iteration $\Delta c = h\mathbf{J}_i$, we can run the setup and get the point cloud $\mathcal{P}_{i+1}^c$. Then we can estimate the Jacobian in the next iteration by
% \begin{equation}
% \mathbf{J}_{i+1} = \mathbf{J}_{i} + \Delta \mathbf{c}^T \frac{\Delta \mathbf{o} - \mathbf{J}_i \Delta \mathbf{c}}{\Delta \mathbf{c}^T \Delta \mathbf{c}}
% \end{equation}
% In the estimation process, the objective function is represented by a vector $\mathbf{o}$, which computed by the positions difference of control points in a particular block region on the fitted B-spline surface. Here $\mathbf{o}$ is written as
% \begin{equation}
%     \mathbf{o}^T = [||(\mathbf{R}\mathbf{p}_{1,1}^t + \mathbf{t}) - \mathbf{p}_{1,1 }^c||, ..., ||(\mathbf{R}\mathbf{p}_{b,h}^t + \mathbf{t}) - \mathbf{p}_{b,h}^c||] \in \mathbb{R}^{bh}
% \end{equation}
% and therefore $\Delta \mathbf{o} = \mathbf{o}_{i+1} - \mathbf{o}_{i}$. As a approximation method, we remark the Jacobian computed by this method as $\mathbf{J}_{est}$, which is run in each iteration after the initial guess.

% \begin{align}
%       T=
% \left[
%  \begin{matrix}
%   {Q(1,1)-Q_{target}(1,1)}\\
%   {Q(1,2)-Q_{target}(1,2)}\\
%   ....\\
%   {Q(n_i,n_j)-Q_{target}(n_i,n_j)}
%   \end{matrix}
%   \right]
% \end{align}

% where the pseudoinverse of the Jacobian $\mathbf{J}^*$ can be estimate using same method as well. For each iteration loop, after getting the Jacobian matrix for current status, we can detect the best update step by line-search method~\cite{} that the actuation parameter in the next iteration as 
% \begin{equation} \label{eq:updateActuation}
%     \textbf{c}_{i+1} = \textbf{c}_i - \mathbf{J}^*\mathbf{o}(\textbf{c}_i)
% \end{equation}


% As a approximation method, $\mathbf{J}_{est}$ can have numerical error \Guoxin{where might be the error comes from?} therefore we can test if the objective value is reduced. If we have $\mathcal{O}(\mathbf{c}_{i+1}(\mathbf{J}_{est})) > \mathcal{O}(\mathbf{c}_{i})$ we will recall (\ref{eq:numericalJacobian}) to update the Jacobian and update the current status. We summary the above process in Algorithm~\ref{alg:shapeControl}.
% .

% .

% .

% \subsection{Step estimation of Gradient-decent optimization}

% .

% .

% .

% \subsection{Preparation of Control Point}

% We remark the mannequin model with mesh representation as $\mathcal{M}$. The control goal is finding the control parameter (represented by vector $\mathbf{c} \in \mathbb{R}^m$) that makes the shape close to given target model shape $\mathcal{M}_t$. As Jacobian-based method is invited in our system, the Jacobian matrix $\mathbf{J} \in \mathbb{R}^{m \times n}$ needs to be computed and updated for each iteration. 

% Here $n$ is the dimention of the control parameters, which can be intuitively set as the coordinate of each vertex in the given target shape mesh $\mathcal{M}_t$. However, this can easily cause a large dimension that requires extreme high computation cost. Instead, in our method we invite the B-spline surface fitting to down-sampling the 
% control variables into the b-spline surface control point, where the target and our current mesh are both fit with same dimension (as detailed in sec...). Therefore, the deformable surface shape $\mathcal{M}$ can be describe as:
% \begin{equation}
%     \mathbf{p}(u,v) = \sum_{i=0}^b \sum_{j=0}^h N_{i,p}(u) N_{j,q}(u)\mathbf{p}_{i,j}
% \end{equation}
% where the $N(\cdot)$ are B-spline basis functions of degree p and q, respectively. The control point position $\mathbf{p}_{i,j}$ is the actual value controlled in configuration space, which lower the dimension with $n = 3bh$. Meanwhile, 

% With this method, we illustrate the difference between two mesh as an objective function which computes
% \begin{equation} \label{eq:objective}
%     \mathcal{O}(\mathcal{M}_t,\mathcal{M}_c) = \sum_{i=0}^b \sum_{j=0}^h || \mathbf{p}_{i,j}^t - \mathbf{p}_{i,j}^c ||_F^2
% \end{equation}
% To best mimic the difference between two deformed status of the surface, we invite ICP to apply the rigid transformation to $\mathcal{M}_t$ and make it close to the current status. We can compute $\mathcal{M}_t^{r} = \mathbf{R}\mathcal{M}_t + \mathbf{t}$ and brings it to (\ref{eq:objective}).



% \Guoxin{Working on the algorithm now}









% Here we invite two 

% When give the initial control vector and shape status ($\mathbf{c}_0$ and 


% input of our method is the target shape model $\mathcal{M}_t$. We define the configuration space control parameter as 

% .

% .

% .

% .

% \newpage


% \Guoxin{The main discussion is, what's the advantage of using Jacobian-based method compare with method of direct distance matching? In the result section we need also add comparison data. My sense is the Jacobian-based method can ensure? the iteration converge in limited time.}

% From design aspect, our mannequin / soft deformable surface combine both soft chamber and linear motor inside, which makes a continue surface with high comparability and external force. Meanwhile we can enrich the working space that enables target shape with large variation.

% Advantage of our method (control aspect): combing Jacobian-based close-loop control, ICP reconstruction and B-spline fitting:
% \begin{itemize}
%     \item The Jacobian method can have fast iteration speed, however to compute singe J by numerical difference is time consuming. (compare with \cite{Stanley16_ICRA}) \Guoxin{Here requires comparison} 
%     \item Our method can support high-dimention surface control rather than single/multiple point control (dimention of our method is higher)
%     \item We invite the ICP reconstruction in the loop that can automate the surface input as well as explore higher the \Guoxin{need discussion here.}
% \end{itemize}

% \Guoxin{above are the method we use and should be mention in our introduction section.}

% 

==> tex/textHybridSolver_withoutConstraints_.tex <==
\section{Hybrid Solver}
\label{Sec:HybridSolver}
\Jun{algorithm demonstration and critical preparation should be included in later chapter}
In this chapter, we would introduce hybrid solution where we analyze the system from two points of view.
\Jun{In this part, pure gradient-based solution must be compared with hybrid solution to present efficiency by physical simulation. }

\subsection{First solution: gradient-based solver}\label{secGradientBasedSolver}
\Jun{We should mention the solving problem is bi-directional: one to fix transformation, next is to fix actuation}

In Equ.\ref{eq:ProblemDefinition-2}, we formulate the system goal into energy minimization problem at a high level, to be more clear, objective could be calculated as weighting sum of distance between vertex $\mathbf{V}_i$ extracted on the captured surface $\mathbf{S^{'}}$ and closest vertex $\mathbf{V}_i^{*}$ on the target surface $\mathbf{T^{''}}$ (orientation and position has been adjusted by $(\boldsymbol{R}, \boldsymbol{t})$). 
\Jun{Should we mention Hausdorff distance?}

  %constrained problem
     \begingroup
    \small
    \begin{equation}
    \label{energyMinimizationProblem}
    \begin{aligned}
    %\underset{\theta }{\text{\theta}} %f(\theta)=$\sum_{i=1}^{n}(x_i(\theta)-x_i^*)^2
    \min_{ \boldsymbol{\textbf{a}}} \quad & 
    E(\boldsymbol{\textbf{a}})=  \sum_{i=1}^{m}{\omega_i^2\{\mathbf{V}_i(\boldsymbol{\textbf{a}})-(\boldsymbol{R}\mathbf{V}_i^*+\boldsymbol{t})\}^2}\\
    \textrm{s.t.} \quad & 
    \textbf{a}_{i_{min}}<\textbf{a}_{i}<\textbf{a}_{i_{max}} \\
       \quad & i=1,2,...,n                 \\
      \end{aligned}
    \end{equation}
    \endgroup

% \par For the purpose of clarity, we would ignore actuation constraints in this chapter and focus on introducing our algorithm, while the hybrid solver with constraints would be demonstrated next chapter.

Considering constraints of actuation, we could find out all of them are linear and inequality. \textit{Interior Point Method} (IPM) is adopted to handle these inequality constraints. That is, treat linear inequality constraints as penalty or barrier into the objective function, and this kind of barrier should satisfy all of the following terms:
\begin{itemize}
    \item Nearly infinity near constraints
    \item Almost zero away from constraints
    \item $C^2$ continuity in order to get gradient and hessian
\end{itemize}

In short, we could adopt functions from natural logarithm family to satisfy these three requirements, and transfer inequality actuation constraints into additional barrier energy term into our objective function:

\begin{equation}\label{Equ: barrierEnergy}
\boldsymbol{I(u)} = -\frac{1}{t}*\ln \left(-u\right)
\end{equation}


When talking about $\mathbf{a}_{i}-\mathbf{a}_{i_{max}}<0$ and $\mathbf{a}_{i_{min}}-\mathbf{a}_{i}<0$, we could replace $u = \mathbf{a}_{i}-\mathbf{a}_{i_{max}}$ and $u = \mathbf{a}_{i_{min}}-\mathbf{a}_{i}$ respectively. We use $k(\mathbf{a})$ to represent these two notations.

\label{modifiedStatement}
Considering barrier energy term, the minimization problem should be rewritten into:
 \begingroup
    \small
    \begin{equation}
    \label{Equ: modifiedObjective}
    \begin{aligned}
    %\underset{\theta }{\text{\theta}} %f(\theta)=$\sum_{i=1}^{n}(x_i(\theta)-x_i^*)^2
    \min_{ \boldsymbol{\mathbf{a}}} \quad & 
    E_{con}(\boldsymbol{\textbf{a}})=\sum_{i=1}^{m}{\omega_i^2 \{\mathbf{V}_i(\boldsymbol{\mathbf{a}})-(\boldsymbol{R}\mathbf{V}_i^*+\boldsymbol{t})\}^2}+\sum_{i=1}^{2n}{\boldsymbol{I_{i}(k(\mathbf{a}))}}\\
      \end{aligned}
    \end{equation}
\endgroup

\par Gradient-based method could be applied here to minimize the objective, and the gradient could be acquired by solving equation defined in Equ.\ref{gradientf} and Equ.\ref{gradientComponentf}.
After getting the gradient of objective function, we take a step in the gradient direction by searching a proper step
size  $\alpha$  with a soft line search method proposed in \cite{9082704}. Then, we could reach next actuation by following equation:

\begin{equation}
\label{updateActutation: gradient descent}
\begin{aligned}
  \boldsymbol{\textbf{a}_{t_{k+1}}} = \boldsymbol{\textbf{a}_{t_{k}}} - \alpha*\nabla E_{con}(\boldsymbol{\textbf{a}_{t_{k}}})
\end{aligned}
\end{equation}

In order to estimate gradient information, we need to update one actuation for each component $\frac{\partial E_{con}}{\partial  \textbf{a}_{i}} $, and if the length of actuation vector is $n$ , so overall frequency of updating actuation for each gradient estimation would be $n+1$ times per gradient (In our setup, these two numbers are 8 and 9 respectively).  What's more, time used to wait for the stability of camera and actuation system dominate the most part of time consumption. So, we turn to look at this problem from another perspective of root-finding problem and invite new method which could accelerate the iteration by reducing the gradient estimation cost. 



\subsection{Second solution: Jacobian-based solver}
\label{secJacobian-basedDescription}

\par Considering the efficiency problem existing in the gradient-based solver, we apply another method called Jacobian-based solver aimed to solve problem stated as following:

\begin{equation}
\label{root-findingProblem}
% \quad for space
% & for alignment
% \\ for new line  
\begin{aligned}
     \textrm{Solve} \quad &  \mathbf{F}(\boldsymbol{\textbf{a}}) =
\left[
 \begin{matrix}
    F_1 \quad F_2 \quad \ldots \quad F_k
  \end{matrix}
  \right]^{T}
   =  \boldsymbol{0}\\
   \textrm{where} \quad & F_j = \sum_{i\in G_j}\omega_i^2\{\mathbf{V}_{i}(\boldsymbol{\textbf{a}})-(\boldsymbol{R}\mathbf{V}_i^*+\boldsymbol{T})\}^2
  \\
  \textrm{s.t.} \quad & 
 \textbf{a}_{i_{min}}<\textbf{a}_{i}<\textbf{a}_{i_{max}} \\
             \quad & i=1,2,...,n                 \\
\end{aligned}
\end{equation}



%{\sum_{i\in c_k}\omega_i^2\{x_{i}(\boldsymbol{\textbf{c}})-(\boldsymbol{R}x_i^*+\boldsymbol{T})\}^2

%%backup of equation
% \begin{equation}
% \label{root-findingProblem}
% \begin{aligned}
%      Solve \quad &  \mathbf{F}(\boldsymbol{\theta}) =
% \left[
%  \begin{matrix}
%   {\sum_{i\in c_1}\omega_i^2\{x_{i}(\boldsymbol{\textbf{c}})-(\boldsymbol{R}x_i^*+\boldsymbol{T})\}^2}\\
%   \sum_{i\in c_2}\omega_i^2\{x_{i}(\boldsymbol{\textbf{c}})-(\boldsymbol{R}x_i^*+\boldsymbol{T})\}^2\\
%   \vdots\\
%   {\sum_{i\in c_k}\omega_i^2\{x_{i}(\boldsymbol{\textbf{c}})-(\boldsymbol{R}x_i^*+\boldsymbol{T})\}^2}
%   \end{matrix}
%   \right]
%   & = \left[ \boldsymbol{0} \right]\\
%   \\
%   \textrm{s.t.} \quad & 
%  \textbf{c}_{i_{min}}<\textbf{c}_{i}<\textbf{c}_{i_{max}} \\
%              \quad & i=1,2,...,n                 \\
% \end{aligned}
% \end{equation}

Each component of $\mathbf{F}$ could be written as $F_{i}$ which represents the sum of distance error of point group $G_i$  comprising of neighbour points around chamber $i$ on captured shape $\mathbf{S^{'}}$. 

\par Similar to what we have done in handling actuation limits in \ref{secGradientBasedSolver}, we add extra energy term in each component of $\mathbf{F}$ as following:

% \quad for space
% & for alignment
% \\ for new line  
% \footnotesize 
\begin{equation}
\begin{aligned}
\label{root-findingProblem:modified-2}
\textrm{Solve} \quad &  \boldsymbol{\mathbf{F_{con}}}(\textbf{a}) =
\left[
 \begin{matrix}
    F_1^{'} \quad F_2^{'} \quad \ldots \quad F_k^{'}
  \end{matrix}
  \right]^{T}
  =  \boldsymbol{0}\\
  \textrm{where} \quad & F_j^{'} = \sum_{i\in G_j}\omega_i^2\{\mathbf{V}_{i}(\boldsymbol{\textbf{a}})-(\boldsymbol{R}\mathbf{V}_i^*+\boldsymbol{T})\}^2 
  \\ & \quad \quad + \sum\limits_{j\in c_j}\{\boldsymbol{I_j(k(\textbf{a}))}\}
\end{aligned}
\end{equation}


First, Jacobian matrix from this perspective could be written as following:
\begingroup
\begin{equation}
\label{jacobian}
\begin{aligned}
    \mathbf{J}^{'}  = \frac{\partial \mathbf{F}^{'}}{\partial  \boldsymbol{\textbf{a}}}=
    \Large
\left[
 \begin{matrix}
   \frac{\partial F_1^{'}}{\partial  a_1} & \frac{\partial F_1^{'}}{\partial  a_2}  &...\\
   \vdots&\ddots&\\
   \frac{\partial F_m^{'}}{\partial  a_1} &  & \frac{\partial F_m^{'}}{\partial  a_n}
  \end{matrix}
  \right]
\end{aligned}
\end{equation}
\endgroup

\begin{equation}\label{BroydenIteration-con}
\boldsymbol{\textbf{a}_{t_{k+2}}} = \boldsymbol{\textbf{a}_{t_{k+1}}} - \beta * \mathbf{J}_{t_{k+1}}^{' -1} \mathbf{F^{'}_{t_{k+1}}}
\end{equation}

\par Equ.\ref{BroydenIteration} represents the iteration of Jacobian-based solver. Here, $\beta$ is a coefficient used to adjust the ratio of step size. The smaller value it is, it represents the conservative attitude towards iteration.

As for how to approximate Jacobian matrix efficiently, Broyden Updating (\Jun{Reference here}) is adopted as following:

\begin{equation}\label{Update}
\mathbf{J}^{'}_{t_{k+1}} = \mathbf{J}^{'}_{t_{k}} +  \frac{\Delta \mathbf{F^{'}_{t_{k+1}}} - \mathbf{J^{'}_{t_{k}}} \Delta \boldsymbol{\textbf{a}_{t_{k+1}}}}{\Delta \boldsymbol{\textbf{a}_{t_{k+1}}}^T \Delta \boldsymbol{\textbf{a}_{t_{k+1}}}}\Delta \boldsymbol{\textbf{a}_{t_{k+1}}}^T
\end{equation}
Where ${ \Delta \mathbf{F^{'}_{t_{k+1}}} = \mathbf{F^{'}_{t_{k+1}}} - \mathbf{F^{'}_{t_{k}} }}$ and 
$\Delta \boldsymbol{\textbf{a}_{t_{k+1}}} = \boldsymbol{\textbf{a}_{t_{k+1}}} - \boldsymbol{\textbf{a}_{t_{k}}}$. 

\par In this updating formula, Jacobian matrix of this iteration is based on the actuation and visual information of this iteration, plus the Jacobian matrix, actuation and visual information of last iteration.

Considering we should calculate the inverse of Jacobian matrix for each iteration if using Equ.\ref{Update}, another updating formulation which is to directly update the inverse of jacobian matrix is written as following: 
\begin{equation}\label{InverseUpdate}
\mathbf{J}_{t_{k+1}}^{'-1} = \mathbf{J}_{t_{k}}^{'-1} +  \frac{ \Delta \boldsymbol{\textbf{a}_{t_{k+1}}} - \mathbf{J}_{t_{k}}^{'-1} \Delta \mathbf{F^{'}_{t_{k+1}}} }{\boldsymbol{\textbf{a}_{t_{k+1}}}^T \mathbf{J}_{t_{k}}^{'-1} \Delta \mathbf{F^{'}_{t_{k+1}}}} \Delta \boldsymbol{\textbf{a}_{t_{k+1}}}^T \mathbf{J}_{t_{k}}^{' -1}
\end{equation}


In the experiments, we adopt the direct updating of inverse of Jacobian matrix instead of calculating inverse matrix each iteration.

\subsection{Comparison of two solutions}
\par Jacobian estimated method from above equations described in \ref{secJacobian-basedDescription} is highly efficient, however, it would not guarantee all the iterations would converge, which means we ought to not just apply Jacobian-based solution.
On the other hand, even if gradient-based method would take us lots of time to execute, the gradient approximated from it would guarantee the incoming iteration would be at least not increase the total objective while running. In short, we would combine these two methods together to formulate our algorithm to leverage convergence of gradient-based method and efficiency of Jacobian-based method (Broyden Updating).

%%Hybrid Solver
\subsection{Solver for hybrid method}
\label{Hybrid Solver}

%Algorithm diagram
\begin{figure*}[t] 
\centering
\includegraphics[width=0.85\linewidth]{fig/workflow-1.png}
\Jun{Algorithm and This flow chart: how to arrange them: maybe this fig is suitable for demonstrating details, and that algorithm description is suitbale to show the high-level logistics.}
\caption{Work flow of first phase of hybrid solver : appropriately arranges gradient-based method, jacobian-based method and registration to generate actuation vector ${\mathbf{a}}$ to deform mesh close to target surface shape.
}\label{fig:solver}
\end{figure*}

The overall algorithm of hybrid solver would be thoroughly presented in two phases. First phase is set to handle actuation limits and achieve fast iteration, while second phase is to achieve real convergence. The main difference between two phases is the objective: the first objective is constraint-involved one, while the second one is original.



% \subsubsection{Estimation of gradient and jacobian matrix}

% \Jun{Should I provide transformation between J and gradient? Maybe too detail...}

% In the hybrid solver, we shall estimate gradient by forward difference using Equ.\ref{gradientf} and Equ.\ref{gradientComponentf}. After that, Equ.\ref{updateActutation: gradient descent} is applied once to reach next step.
% %%gradientComponentf gradientf
% \par Once we finish one gradient-based iteration, we switch to Jacobian-based iteration. The information we acquired in last gradient-based iteration could be used in calculating Jacobian matrix (of last iteration) according to Equ.\ref{jacobian} term by term. Then by Equ.\ref{InverseUpdate} we could estimate the inverse Jacobian matrix of this iteration.

\subsubsection{First phase of hybrid solver}
First phase of hybrid solver is set to achieve fast iteration towards convergence and handle actuation constraints. 
Fig.\ref{fig:solver} illustrates the work flow. It takes target mesh, initial actuation and initial ICP as input, runs iteratively by method 1 (gradient-based solver) or method 2 (Jacobian-based solver) with registration in the loop to get deformed shape near convergence which will be nice initial step for second phase of hybrid solver to proceed to convergence.

\subsubsection{Second phase of hybrid solver}
Second phase of hybrid solver is to achieve real convergence considering only shape difference between target shape and deformed shape as objective. 
\par Naturally, we would meet the situation when actuation proceeds to boundary. In order to handle this stuff, we adopt projection-based method to modified gradient. First, we should judge which actuation reach the check line of actuation constraint:

\begin{equation}
a_{i_{check}} = \begin{cases} 
      a_{i_{max}} - \Delta a_{i}& i\in K_1\\
      a_{i_{min}} + \Delta a_{i} & i\in K_2 
   \end{cases}
\end{equation}

Here, $K_1$ is the set of all maximum constraints, while $K_2$ is the set of all minimum constraints. If the actuation is between check line and actuation constraints, it will be marked as the actuation violating check line.

Considering gradient $\nabla E = [\frac{\partial E}{\partial  a_{1}},\frac{\partial E}{\partial  a_{2}},...,\frac{\partial E}{\partial  a_{n}}]^{T}$, we keep initial gradient vector length and redistribute this length to all actuation which doesn't violate check line donated by set $\textbf{C}$. The modified gradient should be written as following way: 
% \begin{equation}
% \label{gradientProjection}
% \begin{aligned}

% % \frac{\partial E}{\partial  a_{i}} 
% % = 
% \end{aligned}
% \end{equation}

\begin{equation}
(\frac{\partial E}{\partial  a_{i}})_{m} = \begin{cases} 
\frac{\norm{\frac{\partial E}{\partial  a_{i}}}} 
{\sqrt{\sum\limits_{j \in \textbf{C}} \norm{\frac{\partial E}{\partial  a_{j}}}^2}} \norm{\nabla E}
          
          & i \in \textbf{C} \\
          \quad \quad \quad \quad 0 & i\notin \textbf{C} 
\end{cases}
\end{equation}


After getting modified descent direction $\nabla E_{m} = [(\frac{\partial E}{\partial  a_{1}})_{m},(\frac{\partial E}{\partial  a_{2}})_{m},...,(\frac{\partial E}{\partial  a_{n}})_{m}]^{T}$, we proceed to next actuation by appropriate step size defined as:
\begin{equation}
\label{updateActutation: gradient descent}
\begin{aligned}
  \boldsymbol{\textbf{a}_{t_{k+1}}} = \boldsymbol{\textbf{a}_{t_{k}}} - \alpha*\nabla E_{m}(\boldsymbol{\textbf{a}_{t_{k}}})
\end{aligned}
\end{equation}


%%%Algorithm%%%%%%%%%%%%
%\begin{comment}
\Jun{Should modify objective: variable should include R and t.}
\begin{algorithm}[t]\label{alg:hybridSolver}
\caption{Hybrid Solver}

\LinesNumbered

\KwIn{Captured shape $\mathcal{S}^{'}$, target shape $\mathcal{T}^{''}$, initial actuation vector $\mathbf{a_0}$ and the maximally allowed iterations $i_{max}$.}

\KwOut{The actuation parameters $\mathbf{a}$ , rigid transformation ($R$, $t$) and resulted shape $\mathcal{S}^{'}_{\mathbf{a}}$} 

\tcc{First phase of hybrid solver}

Set $i = 0$ and
apply initial actuation vector $\mathbf{a_0}$;


Apply ICP to target shape and get ${(R_{0},t_{0})}$;

Evaluate the objective function $E^{'}_0 = E^{'}(\mathbf{a}_0,R_{0},t_{0})$;

%Compute initial ${\nabla f_{t_{0}}}$ and $\mathbf{J}_{t_0}$ by numerical differentiation (Equation \ref{gradient} and \ref{jacobian}).

\While{$E_i^{'} > \lambda$ {or $i<i_{max}$}}{
\tcc{Gradient-based solver}
Compute initial ${\nabla E^{'}_i}$ and $\mathbf{J}^{'}_{i}$ by numerical differentiation (Equ.\ref{gradientComponentf} and Equ.\ref{jacobian});

Cal step size $\alpha$ and update $\mathbf{a_{i+1}}$ by Equ.\ref{updateActutation: gradient descent};


Run $\mathbf{a_{i+1}}$ in physical setup and generate $\mathcal{S}^{'}_{i+1}$;

let m = 0 and evaluate the objective function $E^{'}_{i+1+m} = E^{'}(\mathbf{a}_{i+1+m},R_{i},t_{i})$;

% $E_i^{'} > \lambda$ {or $i<i_{max}$}

\tcc{Jacobian-based solver}
\While{$E^{'}_{i+1+m}$ keep decreasing {and $m<m_{max}$} }
{

Update Jacobian matrix by Equ.\ref{InverseUpdate};

proceed to next actuation using Equation \ref{BroydenIteration-con};
    
m = m+1;

Evaluate the objective function $E^{'}_{i+1+m} = E^{'}(\mathbf{a}_{i+1+m},R_{i},t_{i})$;

} 

i=i+1+m;

\If{$E^{'}_{i}$ increases}
{
Roll back to last actuation and mark as $\mathbf{a_{i}}$;
}


\If{i$\mod$k == 0 }
{
Apply ICP to target shape and update ${(R_{i},t_{i})}$;
}
Evaluate the objective function $E^{'}_{i} = E^{'}(\mathbf{a}_{i},R_{i},t_{i})$;
}

\tcc{Second phase of hybrid solver}
\While{$E_i^{'} > \lambda$ {or $i<i_{max}$}}{
\tcc{Gradient-based solver}
Compute projected ${\nabla E_i}$ and $\mathbf{J}_{i}$ by numerical differentiation;

Cal step size $\alpha$ and update $\mathbf{a_{i+1}}$;


% Run $\mathbf{a_{i+1}}$ in physical setup and generate $\mathcal{S}^{'}_{i+1}$;

Evaluate objective $E_{i+1} = E(\mathbf{a}_{i+1},R_{i},t_{i})$;

i = i+1;

\If{i$\mod$k == 0 }
{
Apply ICP to target shape and update ${(R_{i},t_{i})}$;
}
}

\textbf{return} $\mathbf{a}$,  $\mathcal{S}_{a}^{'}$, $R$, $t$;

\end{algorithm}

%\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Algorithm: Hybrid Solver}
In this section, we would explain our optimization algorithm consists of all components explained in the previous sections.
\par In short, we split the optimization solver into two phase:  In first phase, in order to get fast and accurate iteration, we use numerical difference which changes the actuation step by step to get initial gradient 
${\nabla E^{'}(\boldsymbol{\mathbf{a}_{t_{k}})}}$, (At the same time, we calculate the Jacobian matrix ${\mathbf{J}_{t_{k}}^{'-1})}$and then adopt soft line search method to gain step size ${\alpha}$, finally we proceed to next actuation ${\boldsymbol{\mathbf{a}_{t_{k+1}})}}$. At this actuation, we switch to Broyden updating. When energy 
${E^{'}(\boldsymbol{\mathbf{a}})}$ keeps decreasing and broyden iteration doesn't exceed maximum, we stay in Jacobian-based solver. Once we found energy exceeds the former step ,we would roll back to last actuation. Then, we return to gradient-based solver and re-calculate the initial gradient and Jacobian once again. Remember, every k times we re-enter the gradient-based solver, we would use ICP to align current shape and target shape to provide alternative converge direction. The workflow of first phase of hybrid solver could be found in \textbf{Fig} \ref{fig:solver}.
\par In second phase,constraint-involved objective is replaced with the original objective and then gradient-based solver is adopted to execute the iteration to pursuit the real convergence status. All details of hybrid solver could be found in Alg.\Ref{alg:hybridSolver}.


==> tex/textICP-in-the-loop.tex <==
\section{Registration in the loop}
\Jun{Modified in Oct 9}
In this chapter, we would introduce registration implementation in our shape approximation task, and introduce experimental results to validate the necessities and advantages of this strategy.

\subsection{Significance of registration in task}
\par In our project, considering we need to approximate the captured shape to target shape as much as possible, however, it is hard to compute optimal orientation and translation (also called rigid transformation) of target shape relative to current shape from the very beginning. 

\par In \cite{StanleyICRA2016}, manual calibration and complicated initial alignment were conducted  to fix the rigid transformation. This method would be a success if target shape is already in the feasible region or the geometry is simple.

\par On the contrary, rigid transformation should be iteratively revised during iteration to provide better efficiency and approximation results.

\par As a result, Iterative Closest Point Algorithm (ICP) which is a widely used algorithm computing rigid transformation that minimizes the difference of two point clouds has been invited in our solver to handle registration task.




\subsection{Experimental validation of ICP}
\par In this part, some experiments were conducted in 2x2 chamber array (as shown in Fig.\ref{fig:2x2chamberSetup}) to validate the importance of ICP. 

%2x2 chamber array setup
\begin{figure}[t] 
\centering
\includegraphics[width=0.85\linewidth]{fig/ICP-setup.png}
\caption{ICP validation experimental setup: Actuation system, scanner, control center and 2x2-Chamber based membrane.
}\label{fig:2x2chamberSetup}
\end{figure}

\par In the experiment, we actuated the membrane with randomly selected actuation parameters and recorded the surface shape at that moment. After that, we chose this surface shape as target and applied initial rotation which is selected in the set: xy-0°(xz-0°), xy-20°, xy-40°, xy-60°, xz-20°, xz-60°, xz-80°. 
Note that the rotation matrix is  following XYZ-Fixed Angle System. For example, xy-20° means we first rotate captured target shape along x axis then along y axis for 20 degrees separately.
This initial adjust is added here for the purpose:

\begin{itemize}
    \item Create posture misalignment for captured surface and target surface, which could be used to test the role of ICP in our shape approximation algorithm. 
    \item Find the maximum capability of registration to adjust the misalignment in the approximation. As we know, ICP would diverge when misalignment is too severe. 
\end{itemize}

After the initial adjustment was finished, we applied our control algorithm (\ref{Sec:HybridSolver}) to see the role ICP played in the iteration.

\par According to Fig.\ref{fig:2x2chamberEnergy}, we could know ICP algorithm makes control solver in
\ref{Sec:HybridSolver} robust due to the final energy converged to same level. At the same time, ICP dose have its own effective working range: In Fig.\ref{fig:2x2chamberEnergy}(a) and (b), when angle is around 60 degree and 80 degree, the iteration would fall into local minimal rather than decrease to same energy level as others.

\par Reconstructed meshes and distance error colormap during whole iterations would be fully demonstrated to see the shape approximation processes. In Fig.\ref{fig:icpComp1}, two iterations are near the maximum capability of registration reasonably adjusting the target posture with respect to real time mesh. In the first and second row, we could see the shaded mesh and mesh with colormap. With registration in the loop, large error indicated by red could be efficiently eliminated. While in the fourth row, registration couldn't provide suitable posture and iteration stuck in local minimal. In down right corner, we could see some regions in colormap is still red which indicates the matching error is quite high, about more than 15mm. 

\par From the experiments illustrated in mentioned figures, the conclusion that ICP algorithm plays an important role in our solver by gradually adjusting the converging direction of our actuation.

%2x2 chamber array energy
\begin{figure}[t] 
\centering
\includegraphics[width=0.95\linewidth]{fig/fig-2x2ChamberEnergy.png}

\caption{ After applying different initial rotation angles on the target surface, we acquired the energy-iteration figs to compare. (a). We first rotate target shape along x axis, and then y axis to modify the orientation of target before applying control algorithm. (b). Initial rotation consists of one rotation along x axis and then one rotation along z axis.
}\label{fig:2x2chamberEnergy}
\end{figure}

%2x2 chamber array energy comparison
\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/ICP-comprison1.png}
\caption{ Iteration Comparison of Two cases: Initial rotations are XZ-60 and XZ-80 respectively. Note that the second row shows registration still has its own maximum capability, so we should apply ICP within the ability. Note that these meshes are from side view.
}\label{fig:icpComp1}
\end{figure}



==> tex/textIntro.tex <==
\section{Introduction}\label{secIntro}
\Jun{Modified in Oct  11}
\IEEEPARstart{S}{hape} morphing system has the ability to switch the geometric state from one to another by applying several actuation or releasing pre-injected energy\cite{ShapeChangingClassification}, such as unfolding origami structure or inflating the enclosed volume of inflatables. Their applications in medical treatment, garment industry and soft robotics are emerging nowadays. 

% \JunReplace{Deformable surface have the ability of shape changing through controlled actuation, which are nowadays have increasingly application such as 2D/3D haptic system~, soft mannequin~, and shape display~. Current implementation of these surface lies on either pin array actuators~ or continuous fluid/air driven soft chambers~. For both design, a deformable out-layer membranes can be invited to keep a continue smooth surface that best mimic the target shape.}{}
In garment industry, with the popularity of online shopping\cite{unctad_2021} especially in pandemic, the return rate is hugely increased\cite{returnRate}. The main reason is standards would vary according to garment brands and era. Garment manufacturers tend to formulate their own size standard\cite{clifford_2011}\cite{stampler_2014} and people's common dimension would also vary as the society is developing\cite{stampler_2014}. A unknown fact is that a high portion of returned items would possibly end up with landfills leading to tremendous resources wasting and carbon emission\cite{schiffer_2019}\cite{theguardian_2020}. As a result, shape-morphing device as deformable robotic mannequin is proposed targeted on both clients and garment designers to help with this problem. For garment designers, the deformable mannequin could be used to verify and improve their designs covering different body dimensions from just one single robotic mannequin. For individual person, once they acquire scanned data and then could send to cloth store and wait for remote fitting to select the suitable garment without coming to cloth store in person. 
\par However, most of current robotic mannequins are still focusing on relatively rigid material (panel or belt), which could not achieve large local deformation, such as in chest and waist region. This would not cover the most of human body dataset, limiting the application range of their mannequins. 

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{fig/DeformableManneuqin.png}
\caption{Illustration of workflow: soft mannequin made from silicone can be deformed by controlled flow pressure, and its overall shape is captured by high-end scanner. Together with Region of Interest (ROI) selected from human model, we apply proposed algorithm to actuate the captured shape to approximate the target shape.
}\label{fig:WorkFlow}
\end{figure}

This perspective directly brings us a motivation: 
build up a soft robotic mannequin system that could be deformed by pneumatic actuation. Along with low-level pressure control system and vision feedback device, we could control the deformation of soft mannequin to approximate input target models with large variations in soft tissue regions(chest and waist, etc). The overall workflow of this objective is illustrated in Fig.\ref{fig:WorkFlow}. 



%old
% Deformable surface among shape morphing system, can be controlled by pre-defined patterns on the specific location () or sequentially applied actuation (where our paper lies on). The continuous surface variation in 3D surface could mimic different types of target shape which then could be used in many areas. 


% As a deformable object, the continuous surface with large degrees-of-freedom (DOFs) would bring large complexity in the control task. The control for such soft surface is normally described as computing configuration space parameters that can enable the surface/object reach best with target shape. This kind of approximation task is usually defined as under-actuated since the number of actuation is normally smaller than variables used to describe the surface. The currently existing solutions can be divided into two kinds. One is model-based method, usually from numerical-based simulation, where different physical models (e.g. mass-spring~\cite{} and finite-element~\cite{}) is conducted that virtually mimics the behavior of the deformable model. \Jun{Just state methods we know} Another solution is model-free, one of which based on large scale of collected data to train a network describing physical situations. Another is normally implemented by vision-based feedback control where deformation information is directly comes from different kinds of camera. In Vision-feedback aspect, pure-P control is adopted to adjust the actuation(); Also, vision information can be used to form the deformation jacobian which determines the sequential actuaion parameters (). Our algorithm proposed in this paper makes use of vision feedback information to gradually approximate the captured shape into target one.


% \JunReplace{When it comes to gradient-based method, David proposed a model-free method that utilized online Jacobian estimation to accelerate the iteration that gradually manipulated the elastic object to a target shape. However, the target shape of its objectives was relatively simple, which is either 2D curve or 3D curve. On the contrast, in this work we developed a gradient-based method to solve the continuous surface approximation problem by smartly select the Jacobian,either by numerical based method or direct computing.}{}


\subsection{Problem Statement}
In this part, overall working flow will be presented with energy term defined to describe system status, and some basic difficulties of solving actuation optimization problem would also be explained.
\subsubsection{Overall Workflow Introduction}
\Jun{Here, should be modified according to revised fig1}
\par Our paper presents an optimization solver to actuate the soft and continuous membrane to approximate Region of Interest (ROI) from female body, and fig.\ref{fig:WorkFlow} shows the main diagram of work flow through following steps:
\begin{itemize}
    \item A display system that includes soft membrane (actual surface shape could be described as $\mathbf{S}$) placed above several chambers can be largely deformed by actuation vector $\mathbf{a}$ including chamber inflation($\mathbf{P_{i}}$) and linear displacement($\mathbf{L_{i}}$) of each chamber .
    \item One female model is generated and partially selected to be ROI, and then served as target surface ($\mathbf{T}$). While actual membrane shape $\mathbf{S}$ could be captured by high-end scanner and processed by B-Spline Surface fitting to be fitted surface shape $\mathbf{S^{'}}$.
    
   
    \item Target fitted surface shape $\mathbf{T^{''}}$ could be generated from target surface shape $\mathbf{T}$ and applied rigid transformation $RT(*)$ to better align with fitted captured surface $\mathbf{S^{'}}$.
    
     \item Consider  the shape difference (between $\mathbf{S^{'}}$ and $\mathbf{T^{''}}$) as objective to be minimized, our proposed algorithm (including updating rigid transformation when appropriate) would automatically generate actuation vector $\mathbf{a}$ to reduce the objective. 
    % \item Actual membrane shape $\mathbf{S}$ could be captured by high-end scanner and processed by B-Spline Surface fitting to be fitted surface shape $\mathbf{S^{'}}$, along with fitted target surface $\mathbf{T^{''}}$ (approximation of target shape $\mathbf{T}$),
    % \item A series of actuation vector $\mathbf{a}$ could be calculated from our proposed algorithm and applied on the physical hardware setup to minimize the shape difference between $\mathbf{S^{'}}$ and $\mathbf{T^{''}}$.
    \item After several iterations, the captured shape $\mathbf{S^{'}}$ would be much more similar to target shape $\mathbf{T^{''}}$.
\end{itemize}

%%%%%Difficulties in solving problem
%why it is hard to minimize the energy function
\subsubsection{The difficulties of continuous shape approximation}
\par In general, the optimization task of this continuous shape approximation could be stated as energy minimization problem where the energy describes the difference between captured fitted surface $\mathbf{S^{'}}$ and target fitted surface $\mathbf{T^{''}}$:


% \begin{equation} \label{eq:ProblemDefinition-1}
% E = \sum_{i\in \textbf{S}}\omega_i D(\mathbf{V}_i(\textbf{c}), R\mathbf{V}_i^{'}+t).
% \end{equation}

\begin{equation} \label{eq:ProblemDefinition-2}
E =  \mathbf{D}(\mathbf{S^{'}}(\textbf{a}), RT(\mathbf{T^{''}})).
\end{equation}


\par As shown in Equ.\ref{eq:ProblemDefinition-2}, $ D(*,*) $ measures shape difference of two freeform surface. In order to ensure the feasibility of approximation, extra DoFs have been applied to target shape $\mathbf{T^{''}}$ by implementing rigid transformation $ (R, t) $ donated by fuction $RT(*)$. Note that captured shape $\mathbf{S^{'}}$ could be deformed by actuation parameter vector $\textbf{a}$. Considering minimizing energy defined in Equ.\ref{eq:ProblemDefinition-2}, some difficulties could be summarized as following:
\begin{itemize}
\item High non-linearity: The relationship between membrane shape $\mathbf{S^{'}}$ and actuation vector $\mathbf{a}$ is highly nonlinear which means the small variation of actuation vector  ($\mathbf{\triangle a}$) would lead to different variation of membrane shape ($\mathbf{\triangle S^{'}}$) when actuation vector $\mathbf{a}$ changes from one to another.

\item  \Jun{Maybe discuss later...Why not simple IK problem? definition of IK}Energy defined in Equ.\ref{eq:ProblemDefinition-2} is involved with rotation and translation which makes our problem not a simple Inverse Kinematics (IK) problem. Instead, Iterative Closest Point (ICP) algorithm is adopted to gradually find the suitable orientation and position of target membrane $\mathbf{T^{''}}$ with respect to captured shape $\mathbf{S^{'}}$.
\item No priori knowledge about mechanical property of chamber and membrane: The cost to calibrate the elastic parameters of chamber and membrane is high, and it is also hard to model the interaction between chamber and membrane.

\item Cost to get gradient is too high: the gradient of energy could be written as following:

\begin{equation}
\label{gradientf}
\begin{aligned}
  \frac{\partial E}{\partial  \textbf{a}_{i}} = \frac{E(...,\textbf{a}_{i}+\Delta \textbf{a}_{i} ,...)-E(...,\textbf{a}_{i},...)}{\Delta \textbf{a}_{i}}
\end{aligned}
\end{equation}

\begin{equation}
\label{gradientComponentf}
\begin{aligned}
  \nabla E = [\frac{\partial E}{\partial  \textbf{a}_{1}},\frac{\partial E}{\partial  \textbf{a}_{2}},...,\frac{\partial E}{\partial  \textbf{a}_{n}}]^{T}
\end{aligned}
\end{equation}

So if we apply gradient-based method, then we need to update n+1 actuation vector $\mathbf{a}$ to get the gradient information, which would take lots of time. In order to solve this problem, we come up with hybrid solver to tackle this problem, and details could be found later.
\Jun{Exact chapter of hybrid chapter reference should be added later.}

\item Under-actuated system: In our setup, length of actuation vector $\mathbf{s}$ is much smaller than DoFs used to describe captured shape $\mathbf{S^{'}}$ and target shape $\mathbf{T^{''}}$, so it is impossible to deform captured shape $\mathbf{S^{'}}$ to match target shape $\mathbf{T^{''}}$ without error, which could be called under-actuated system. In this situation, error is inevitable, and we could only decrease the error as much as possible. The details of handling this stuff could be found later.

\Jun{Exact chapter of grouping critical points could be found later.}
\end{itemize}



\subsection{Contribution of this paper}
\Jun{Modified in Oct 10}
\par As a summary, the contribution of our paper includes follows aspects.
\begin{itemize}
    \item   This is the first completed soft robotic mannequin system driven by injected air including design, fabrication and close-loop shape control. 
    
    \item The novel chamber based design allows large local deformation and outer membrane enables overall smooth shape. Our fabrication methods are able to generate soft curved chambers (silicone) bonding with rigid material (PLA) tightly without air-leaking problem. 
    
    %old 
    % a limited number of actuation (linear rods and air chambers) which could achieve large operation space and approximate ROI of different human bodies.
    
    %old
    % \item Model-free vision-based method is used in surface approximation, which to the best of our knowledge has not been realized by others in real physical setup.
    
    \item We have achieved vision-based close-loop shape control of soft mannequin from one template models to approximate several target models. The shape control method is model-free which means we don't need the exact material property of silicone rubber and contact property between different materials.
    
     \item Registration is invited in the actuation optimization loop to provide extra Degree-of-Freedoms (DoFs) to reduce the shape difference between captured shape and target shape. This registration-in-the-loop strategy fills the gap between virtual model and physical output.
     
    % \item The proposed working pipeline which controls the continuous shape deformation could be applied in garment industry (especially in stem ironing and cloth try-on) without building several prototypes according to the dimension of different customers which could hugely reduce the time and resource cost.
\end{itemize}

We conducted experiments using not only digital platform but also physical setup to verify the behavior of our design and control method, which allows the soft robotic mannequin to deformed towards a variety of target shapes in our implementation.






 

==> tex/textMinimizationDetail.tex <==
% \section{Implementation details}
% \Jun{This should comprise of feature point preparation, high-level workflow and hardware system }
% In this chapter, minimization details of complete control algorithm would be represented, including actuation range balancing, constraints and constraints-involved solver to handle actuation range limits.

% \subsection{Actuation Range Balancing}
% \par In machine learning, in order to get high-quality dataset, we need to apply feature scaling to have several features compatible in range. Also, in our experiments, actuation range of pressure is [0, 20] KPa which is highly different from that of rod linear displacement ([0, 7500] Cycle). When applying hybrid solver, we should apply range balancing so as to acquire normal iteration results.
% \par As for where and how we apply range balancing, please note that the core of range balancing is to influence gradient and jacobian, so the place we should apply range balancing is:

% \begin{itemize}
% \item Before calculating gradient by Equ.\ref{gradientComponentf} and jacobian by Equ.\ref{jacobian}, we should shrink the rod linear displacement by certain ratio. 
% \item When next actuation needed to be calculated, inverse ratio should be applied to rod linear displacement to get correct actuation in Equ.\ref{updateActutation: gradient descent} and Equ.\ref{BroydenIteration}.
% \end{itemize}

% \par Note that the ratio in our experiment is  $ \frac{1}{300} $.

% % \subsection{Preparation of feature points}


==> tex/textRelatedWorks.tex <==
\section{Related Work}

There are several topics related to our paper: shape display with morphing, robotics mannequin and close-loop control of soft robotics. In the following pages, related works about these topics would be reviewed in detail. 

% \begin{figure*}[h]
% \centering
% \includegraphics[width=\linewidth]{fig/ViconSetup.png}
% \caption{ (a) An overview of the soft deformable surface setup and the vision feedback system using Vicon motion capture cameras. (b) Details of hardware setup including
% control unit (microcontroller and multi-stepper driver), actuation unit (syringer and push rod) and display unit (chamber array with covered membrane). (c) Side view of actuation unit including push rod and chamber. With the movement of rod and inflation of chamber, setup could provide large deformation and small features. \Guoxin{Figure will be updated later}\Jun{Will be polished later}
% }\label{fig:systemOverview}
% \end{figure*}

% \subsection{Design of deformable surface}

%\Guoxin{A table should be listed here to compare our design with current exist design}
\subsection{Shape display with morphing}
\Jun{Modified in Oct 9}
\par Shape morphing defined as geometry details could be switched from one to another. In this part, we could go through researches from two aspects: without and with actuation.
\subsubsection{Shape morphing without actuation}
First well-known item is origami whose goal is to transform a flat square sheet of paper into a three-dimension character through paper folding without any cuts, glue and even marking. 
Tachi et al. (2010)\cite{OrigamiSurface} proposed an inverse solver which converts a given polyhedral surface into a folding pattern that folds into a given 3D shape. Note that this is the first practical method and system for constructing a 3D origami model. There are several researches are about constructing 3D shape from 2D material.Garg et al. (2014)\cite{WireMeshDesign} developed a computational approach for designing wire meshes, which could be formed as curved surface of complicated 3D object drawn inspiration from the geometric model of Chebyshev nets.
Malomo et al. (2018) \cite{FlexMap} presented a framework fabricated smooth shapes out of flat and flexible panels with tailored mechanical properties. Researchers from GCL of EPFL \cite{BeyondDeployable} built up an non-linear optimization solver to decide the triangle linkage and generate curved surface from flat pieces, which has been applied in architecture\cite{DeployableShell} and surgery\cite{RapidDeployable}. 

\subsubsection{Shape morphing with pressure actuation}
Peele et al. (2019)\cite{UntetheredStretchable} designed and fabricated a soft spherical interface consists
  of air chambers with color to provide both visual and tactile display. Robertson et al. (2019)\cite{Robertson2019ACM} constructed a system made of square grid array of linear vacuum-powered soft pneumatic actuators (linear V-SPAs). This soft actuator array can be used to transport different types of items via shape changing. Festo\cite{wavehandling} introduced WaveHandling: a soft deformable surface covering numerous bellows which could be actuated linearly according to pressure of inflated air. This could be used to transport, caging objects by creating wave-like profiles. Siéfert et al. (2018) \cite{Sifert2018BioinspiredPS} presented shape morphing elastomer embedding a network of airways which are not uniform in the plane, resulting in the an-isotropic deformation. By taking advantage of this characteristics, they built a solver to "decode" the target curved surface into initial airway pattern. When the network inflated, deformed shape is closed to target shape. Ma et al. (2017)\cite{BeatingHeart} presented 3D deformable heart-like object composed of several chambers and frame structures and it would deform to different target shapes. As for computational inverse design of balloon which could be inflated to approximate target shapes, Skouras presented their excellent works in \cite{balloon}\cite{inflatableStructures}. Charm Lab from Stanford conducted some researches in shape display with soft material in \cite{StanleyChamberArray}\cite{StanleySurfaceHaptic}, and later, fully 3D display has been demonstrated in \cite{3Dhaptic}. Sparrman et al. \cite{sparrman} presented their liquid printed pneumatics chamber array which could be inflated to form complicated shape sequences.
  
\subsubsection{Shape morphing with linear movement} 
Basically, the core of projects here is the dense pin array which could be linearly moved up and down to form discretized complicated shape. Works like Project FEELEX(2001)\cite{Iwata2001ProjectFA}, Relief(2010)\cite{Relief}, InFORM(2013)\cite{inForm} and  ShapeShift(2018)\cite{Siu2018shapeShift2S} demonstrate the shape morphing capability. There are outer membrane cover providing continuous overall shape in  \cite{Iwata2001ProjectFA}\cite{Relief}. Je et al. (2021) \cite{Je2021ElevateAW} constructed a high-resolution and walkable pin-array display mimicing different types of physical terrains and the walking experience would be enhanced in virtual reality.

\subsubsection{Shape morphing with other actuation}
Actuation source of shape morphing could be achieved by other actuation excluding pressure and linear movement, like uniform heating\cite{origamiHeating}\cite{Boley20856}, joint toque\cite{Panetta2019XShells} and joint movement\cite{elasticGeodesicGrids}. 


\subsection{Deformable robotic mannequin}
\Jun{Modified in Oct 9}
In garment industry, mannequin is essential for customers to preview the try-on effects especially useful in online shopping. Usually, the mannequin is hard and fixed, so each mannequin is tailored just for one individual person. It is very time-consuming and so deformable mannequin is needed in this scenario. 

Researchers from TalTech conducted a series of researches in rigid mannequin. Abel et al. (2009) \cite{design_shape_changing_mannequin_2009} first built up a shape-changing mannequin targeted on male, then they improved their work by taking female models into consideration\cite{Abels2013ConstructionOA_female_mannequin}. 
Later, shape control of rigid mannequin was realized by establishing a simulation model (Abel et al., 2013\cite{shapeCtrl_mannequin_2013}) . The optimized actuation parameters could be calculated from built simulator and applied on real mannequin model. 

However, only rigid material is adopted in \cite{design_shape_changing_mannequin_2009}\cite{Abels2013ConstructionOA_female_mannequin}\cite{shapeCtrl_mannequin_2013}, leading to small local deformation. As a result, large error would occur around stomach and chest. 

Researchers from ZJU have done similar researches in rigid mannequin. Xu et al. (2018)\cite{hardMannequin} proposed hard deformable mannequin whose shape is controlled by a flexible belt. Simulation results are shown and physical experiments are 
not available. Guo et al. (2018)\cite{Guo2018StructuralDA} proposed a deformable panel-based mannequin with physical prototypes. However, they could not provide quantitative analysis for the approximation result. Note that large local deformation could not be achieved in chest and waist region. Guo et al. (2019)\cite{Guo2019TheDO} proposed an entire remote fitting system included a flexible mannequin proposed in 
\cite{Guo2018StructuralDA}. With these in hand, they could provide try-on effects and comfort information to customers to help reduce the return rate of garment. Li et al. (2021) \cite{JITUOcompMann2021} computationally designed robotic mannequin from human body database, and verified the approximation by simulation and physical experiments.

Researchers from PolyU \cite{polyuDummy} invented i.Dummy, a rigid robotic mannequin to fit different types of people and dimension ranges could be found in \cite{DummySpecification}.

A French fashion company Euveka\cite{euveka_2021} created their deformable robotic mannequin targeted on B2B (fashion company like Chanel and Louis Vuitton), and products are in market.

\par The previous researches and products mainly focused on rigid robotic mannequin, which would of course result to small curvature variation in local regions. So the concept of soft mannequin comes naturally. 
\par Chen et al. (2014)\cite{2014SoftMann_Donghua} proposed the concept of soft mannequin with air chambers on human model. most contents in \cite{2014SoftMann_Donghua} are related to single chamber control, and there are no results about whole shape control and approximation. To the best of our knowledge, there doesn't exist whole system of soft mannequin design, fabrication and shape control. This is also where our project stands. 



\subsection{Close-loop control of soft  robots}
\Jun{Need more literature to improve the paragraph}

\par Close-loop control of soft robots could be classified according to two aspects: Model-based method and model-free method. In model-based aspect, analytical methods which describe the model of soft robots as mathematical formulation are widely used in soft robots area because:
\begin{itemize}
    \item Part of soft robots only consists of simple structures or undergoes simple deformation. \Jun{Provide some examples including constant curvature assumption, piece-wise constant curvature examples and so on.}
    \item In many scenarios, soft robots are invited due to its safety when interacting with human beings and environments because they could naturally and slightly change their shape to be compatible with environment. As such, the accuracy of soft robots is not that critical, so simple assumption is acceptable in many applications.
\end{itemize}
\par Another important method from model-based aspect is numerical method which makes use of iteratively tool with mathematics and physics knowledge to simulate the property (e.g. shape) of soft robots. For example, Finite Element Analysis is usually employed to accurately simulate the real situation of soft robots using given material property, constraints, actuation parameters and so on. However, efficiency of FEM computation is not guaranteed, and what's worse, when soft robot is encountering large deformation, it is highly possible to diverge in enterprise-level FEM software like Abaqus
and Ansys. Also, acquisition of material property is a huge burden in soft robot area not only because it is sometimes highly nonlinear and temperature-dependent or even time-dependent(hysteresis) but also because calibration procedures included are time-consuming. What's worse, due to the inconsistency in material properties and fabrication, re-calibration is always needed before usage of another soft robot fabricated by same means (e.g. 3D printing). Need to be mention that the effectiveness of trained mapping is highly related to quality of collected dataset which may cost lots of time and resources.
\par From model-free aspect, machine learning technique is getting more attention due to some mentioned shortcomings of model-based methods. Machine learning method is deployed in soft robotics area to directly learn the mapping among some variables such as position, velocity, dynamic parameters of robots, its actuation and history actuations. (\Jun{Here, we should provide some ML - FK, ML - IK, ML - dynamic papers}) 
\par Another method from model-free aspect is vision-based method. Stanley (\Jun{reference here}) made use of Kinetic to provide point cloud of surface. With this information, he used pure-P control method which adjusted the respect actuation to compensate the distance error or curvature error. \Jun{Provide more about non gradient-based cases}. Another kind of vision-based method would estimate a local property of material and iteratively proceed to convergence. Without prior knowledge of material property of elastic object, David (\Jun{reference here}) leveraged efficiency of online estimation of jacobian matrix to provide real-time actuation command to manipulate the elastic object to approximate target deformed shape described as the form of 2D points, 3D curves and 2D continuous contour. 



==> tex/textResult.tex <==
\section{Experimental validation}

In order to validate our optimization algorithm, two kinds of experimental platforms are established: one is digital platform while the other one is physical setup. Digital platform is created to conveniently verify our optimization solver without physically tuning the experimental equipment which would significantly save lots of time and resource, while physical setup is eventually built and tested to run our optimization solver to get actuated shape.

The work flow of our experiments are shown in $\textbf{Fig.}$\ref{fig:workflow}. Hybrid solver takes target shape $\textbf{T}^{''}$ and processed deformed shape $\textbf{S}^{'}$ as input to generate actuation parameters, which then would be input of experimental platform: abaqus simulator or physical setup. After getting free-form shape of deformable membrane $\mathbf{S}$, we will check if it meets the condition of converge. If yes, script would stop iteration and output deformed shape. If not, the iteration will continue until converge condition is reached.




\par In this section, we will present all experimental results of free-form surface approximation by implementing proposed solver. On digital platform, python is adopted to call abaqus simulator, post-process deformed mesh, implement our solver. While in physical experiment, all processing algorithms and communication with hardware are with C++ to meet real-time requirements. Our work station is a laptop with 2.6GHz CPU (Intel i7-9750H) and 32G RAM. 

%work flow
\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/experimentDemonstration.png}
\caption{Work flow of our experiments: our hybrid solver would generate actuation vector $a$ to be input of experimental platform: either abaqus simulator or physical setup. Acquired deformed membrane would be post-processed and compared with input target ROI to get objective which should be input of hybrid solver.
}\label{fig:workflow}
\end{figure}

%high-level perspective figure
\begin{figure*}[t] 
\centering
\includegraphics[width=0.7\linewidth]{fig/firstVer-TargetModels.png}
\caption{Template model and target models. (a) Template model which would be deformed to different target models from (b1) to (b4).
}\label{fig:targetFig}
\end{figure*}

% \subsection{Model preparation}
\subsection{Design and Fabrication}
In general, our proposed soft mannequin would be able to approximate different target shapes in the human body database, in order to prove the concept of soft mannequin, we choose several targets as demonstration to present our whole mechanical system and shape control method, while we leave the mannequin optimization for future works.
\subsubsection{Chamber design}
\par As shown in Fig.\ref{fig:targetFig}, there are one template model and four target models chosen from Parametric Human Body Generator\cite{BodyGenerator} and UMTRI\cite{umtri}. We then select certain region in front of body as Region of Interest (RoI) treated as either deformed region or target region (marked by light wireframe). 

\par \Jun{Here, chamber division should be clarified}
\par Fig.\ref{fig:chamberDivision} shows the chamber division of template model consisting of two chest chambers and three waist chambers. Note that the middle waist chamber is linked and attached on upper waist and lower waist chamber to form overall large and smooth shape variation. 

\subsubsection{Solid model generation}
In order to fabricate the models to hold the soft material (silicone), grasshopper\cite{grasshopper} in rhino has been used to generate some micro-structure\cite{ROSSING2020108254} to create the strong bonding between solid material (PLA or resin) and soft material (silicone) as shown in Fig.\ref{fig:SolidModel}(c). All fabricated modules are assemblied together to form the whole mannequin as shown in Fig. \ref{fig:AssemblyModel}. 

\begin{figure}[h] 
\centering
\includegraphics[width=0.8\linewidth]{fig/chamberDivision.png}
\caption{Chamber division illustration. (a) Template model with outer membrane. (b) chamber arrays with outer membrane. (c) Outer membrane. (d) Chamber arrays including two chest chambers and three waist chambers.
}\label{fig:chamberDivision}
\end{figure}

\begin{figure}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/SolidModel.png}
\caption{(a) Assembly of chamber array and model basement. (b) left chest module with lattice structure. (c) Micro bonding structure from different viewpoints. (d) The upper shows the fabricated silicone-based chamber with its mold placed nearby (red represents silicone liquid inlet while blue shows silicone outlet). The lower shows the inflated chamber with air pumped in.
}\label{fig:SolidModel}
\end{figure}

\begin{figure}[h] 
\centering
\includegraphics[width=1.0\linewidth]{fig/AssemblyModels.png}
\caption{ Assembly of the mannequin chambers in MeshLab(a) and through fabrication(b)(c). 
}\label{fig:AssemblyModel}
\end{figure}

\subsection{Experiments on digital platform}
\begin{figure}[h] 
\centering
\includegraphics[width=0.9\linewidth]{fig/FigSimulationPlatform.png}
\caption{ Workflow of simulation platform. 
}\label{fig:DigitalPlatformWorkFlow}
\end{figure}

\begin{figure}[t] 
\centering
\includegraphics[width=0.9\linewidth]{fig/digital-icpImportance.png}
\caption{  pose registration validation experiment: validate the importance of ICP algorithm via two groups: (a) hybrid solver with ICP and without ICP. (b) gradient-based solver with ICP and without ICP. \Jun{Need to update}
}\label{fig:digitalICP}
\end{figure}


In order to validate our design and shape control method, we built up a digital platform with python to run hybrid solver and Abaqus simulation at the same time. The work routine of our digital platform is shown in Fig.\ref{fig:DigitalPlatformWorkFlow}. We built the whole system following server-client model where server runs the hybrid solver and distributes the simulation jobs to several clients which are waiting for tasks, and their communications are with TCP/IP protocol. 

\par By the virtually built experimental platform, we could validate not only our design, but also our approximation solvers by comparing their iteration situation.


\subsubsection{Simulation Details}
\par Finite Element Analysis (FEM) Software Abaqus is adopted to conduct chamber inflation and contact simulations. In abaqus, Nonlinear switch of solver (Nlgeom) is turned on. Hyper elastic material is selected and Mooney-Rivlin model is chosen as published in \cite{SiliconePara}: $C_{10}=125.9\ kPa, C_{01}=-17.9\ kPa$.

\par In the simulation, boundary of curve chambers and outer membrane are fixed, and chambers are actuated by pressure from inner side. Constraint of middle waist chamber boundary with other waist chambers is tie constraint. And The terminate condition for hybrid solver is: ${\frac{\Delta \mathbf{E}}{\mathbf{E}}}<0.08\%$. 

% \par Contact pair of membrane and chamber surface is set to surface-to-surface contact and its contact property of tangential behaviour is frictionless.





\subsubsection{Experiment: importance of pose registration}
In digital platform, one experiment is conducted to verify the critical effect of our pose-registration-in-the-loop strategy. To be more specific, we adopt Iterative Closest Point Algorithm(ICP) as pose registration method during the iteration. In Fig.\ref{fig:digitalICP}, hybrid solver would achieve much smaller shape difference with ICP rather than without ICP. It is the same situation even with gradient-based solver. This experiment demonstrates the pose registration is crucial to reduce the energy level by providing more flexibility (DoFs). 

\begin{figure}[t] 
\centering
\includegraphics[width=0.95\linewidth]{fig/RepeatabilityTest.png}
\caption{
Repeatability validation of hyper-elastic material: silicone rubber from Smooth-on. We applied different actuation sequences to see if the control points could be back to original positions.
}\label{fig: repeatability}
\end{figure} 

\begin{figure*}[h] 
\centering
\includegraphics[width=0.9\linewidth]{fig/All-Iteration.png}
\caption{Efficiency comparison between hybrid solver and gradient-based solver using four different target models. 
}\label{fig:AllIteration}
\end{figure*}

\subsubsection{Experiment: solver efficiency comparison}

Shape differences using different target models are plotted in Fig.\ref{fig:AllIteration}, which shows decreasing details of shape difference including all four target models with two solvers. Note that the x axis represents the time used to conduct simulation which would best mimic the time spent in real physical setup. The distance error colormap shows the final shape approximation error between simulated shape and target shape. Compared with gradient-based solver, hybrid solver demonstrates its efficiency by fast converging speed while the final converged results are similar.
\par In Fig.\ref{fig:AllIteration}(c), the first several iterations have been illustrated with a zoom-in, showing the meaning of each step. From the comparison, the hybrid solver outperforms gradient-based method by efficiently updating its Jacobian matrix.  
\subsubsection{Experiment: hybrid solver result}
\par Fig.\ref{fig:shadedMesh} shows the results of hybrid solver to approximate four different target models from template model, and the shaded meshes on the front represent the deformed shape of FEA simulation outputs. In the figure you could see the large local deformation via chamber inflation.

 

\begin{figure*}[h] 
\centering
\includegraphics[width=0.9\linewidth]{fig/fig-shadedMesh.png}
\caption{Shaded meshes of one original mesh and four different converged approximation results using hybrid solver. From left to right: original template model, deformed template mesh to approximate model 1, model 2, model 3 and model 4.
}\label{fig:shadedMesh}
\end{figure*}




\subsection{Experiments on physical platform}

\subsubsection{Experiment: importance of pose registration}
\Jun{Maybe we should not write it here}


\subsubsection{Experiment: material repeatability validation}
Our steady state solver requires the function mapping the relationship from actuation vector to shape difference value should be not related to time, which means the behavior of the system or the process are unchanging in time. In this experiment, we conducted one experiment to verify the repeatability of silicone rubber made by Smooth-on. 

As shown in Fig.\ref{fig:2x2chamberSetup}, we could see soft membrane made from silicone rubber is being scanned to acquire point cloud which could be further processed by B-spline patch fitting\cite{b-splines} and the control grid made of B-spline control points is drawn by blue points. There are one linear actuator and one pressure actuator under the area of control point array (has been indicated by red box), which means these two actuation could hugely influence the position of six control points.

When talking about the arrangement of the actuation sequence, we applied first actuation (5, 300) where 5 Kpa is the pressure value and 300 is for the linear movement (its unit is not calibrated since it is not critical). Then the second actuation was (7,300), and we waited for several seconds and returned to origin. Then, we repeated this by replacing (7,300) with other actuation vectors decided by anti-clockwise directions.

In Fig.\ref{fig: repeatability}, the repeatability results were quit promising: they were all under 0.5 mm. Some of them were even 0.2 mm (No. 10 and No.18 Control Point). With this experiment, we would say the repeatability of this soft material and scanner is excellent and would be used for further surface reconstruction. 

\subsubsection{Experiment: hybrid solver result}


